Heating in Multi-Layer Targets at ultra-high Intensity Laser Irradiation and the Impact of Density Oscillation

We present a computational study of isochoric heating in multi-layered targets at ultra-high intensity laser irradiation (approx. 10**20 W/cm**2). Previous studies have shown enhanced ion heating at interfaces, but at the cost of large temperature gradients. Here, we study multi-layered targets to spread this enhanced interface heating to the entirety of the target and find heating parameters at which the temperature distribution is more homogeneous than at a single interface while still exceeding the mean temperature of a non-layered target. Further, we identify a pressure oscillation that causes the layers to alternate between expanding and being compressed with non beneficial effect on the heating. Based on that, we derive an analytical model estimating the oscillation period to find target conditions that optimize heating and temperature homogeneity. This model can also be used to infer the plasma temperature from the oscillation period which can be measured e.g. by XFEL probing.

==> Notes.tex <==


